Divide-Then-Aggregate: An Efficient Tool Learning Method via Parallel Tool Invocation

Although current Large Language Models (LLMs) exhibit impressive capabilities, performing complex real-world tasks still requires tool learning. Mainstream methods, such as CoT/ReAct, rely on step-by-step tool invocation to interact with external environments, but they are limited in perceptual scope and lack adequate task-planning capability. To address these limitations, other studies introduce the first Search-based Decision Tree (DFSDT), which still suffers from the high computational cost. In this paper, we introduce a novel parallel tool invocation paradigm, DTA-Llama (Divide-Then-Aggregate Llama). First, we transform traditional tree-based tool search paths into Directed Acyclic Graph (DAG) structure, generating a high-quality parallel tool invocation dataset. The DTA-Llama is then trained on the dataset to learn to iteratively divide the current task into several parallel tool invocation sub-tasks and aggregate the invocation results to decide the next actions. Furthermore, we introduce an efficient inference framework inspired by the Process/Threads mechanism when applying the DTA-Llama to practical tasks. Experimental results show that our approach substantially enhances task performance while reducing token consumption and inference time. Llama2-7B, using our method, is comparable to the official parallel function calling method of GPT-3.5. The relevant code, dataset, and model weights are available at https://corn0205.github.io/

==> figures/cache.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|cccccccccccccc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{I1-Inst.}} & \multicolumn{2}{c}{\textbf{I1-Tool}} & \multicolumn{2}{c}{\textbf{I1-Cat.}} & \multicolumn{2}{c}{\textbf{I2-Inst.}} & \multicolumn{2}{c}{\textbf{I2-Cat.}} & \multicolumn{2}{c}{\textbf{I3-Inst.}} & \multicolumn{2}{c}{\textbf{Average}} \\ \cmidrule(l){2-15} 
\multirow{-2}{*}{\textbf{Method}} & SoPR & \multicolumn{1}{c|}{SoWR} & SoPR & \multicolumn{1}{c|}{SoWR} & SoPR & \multicolumn{1}{c|}{SoWR} & SoPR & \multicolumn{1}{c|}{SoWR} & SoPR & \multicolumn{1}{c|}{SoWR} & SoPR & \multicolumn{1}{c|}{SoWR} & SoPR & SoWR \\
\hline\hline
\multicolumn{15}{c}{\textit{GPT-series}} \\
\midrule 
GPT-3.5 (ReAct) & 53.0 & \multicolumn{1}{c|}{-} & 53.0 & \multicolumn{1}{c|}{-} & 51.2 & \multicolumn{1}{c|}{-} & 37.6 & \multicolumn{1}{c|}{-} & 43.9 & \multicolumn{1}{c|}{-} & 48.6 & \multicolumn{1}{c|}{-} & 47.9 & - \\
GPT-3.5 (DFSDT) & 63.8 & \multicolumn{1}{c|}{58.9} & {\color[HTML]{FE0000} 73.9} & \multicolumn{1}{c|}{65.8} & 65.8 & \multicolumn{1}{c|}{60.1} & 57.1 & \multicolumn{1}{c|}{72.6} & 69.8 & \multicolumn{1}{c|}{68.5} & 69.9 & \multicolumn{1}{c|}{67.2} & 66.7 & 65.5 \\
GPT-3.5 (Parallel) & 64.6 & \multicolumn{1}{c|}{48.5} & 65.0 & \multicolumn{1}{c|}{55.7} & 69.0 & \multicolumn{1}{c|}{54.2} & 54.9 & \multicolumn{1}{c|}{55.7} & 61.4 & \multicolumn{1}{c|}{53.2} & 56.6 & \multicolumn{1}{c|}{50.8} & 61.9 & 53.0 \\
GPT-4 (ReAct) & 54.4 & \multicolumn{1}{c|}{53.4} & 44.1 & \multicolumn{1}{c|}{60.1} & 48.8 & \multicolumn{1}{c|}{52.9} & 50.6 & \multicolumn{1}{c|}{69.8} & 48.9 & \multicolumn{1}{c|}{62.1} & 42.6 & \multicolumn{1}{c|}{54.1} & 48.2 & 58.7 \\
GPT-4 (DFSDT) & {\color[HTML]{FE0000} 69.0} & \multicolumn{1}{c|}{57.1} & 69.6 & \multicolumn{1}{c|}{\color[HTML]{FE0000} 66.5} & 68.1 & \multicolumn{1}{c|}{61.4} & 70.8 & \multicolumn{1}{c|}{73.6} & 68.0 & \multicolumn{1}{c|}{62.9} & {\color[HTML]{FE0000} 76.0} & \multicolumn{1}{c|}{63.9} & {\color[HTML]{FE0000} 70.3} & 64.2 \\
GPT-4 (Parallel) & 62.9 & \multicolumn{1}{c|}{\color[HTML]{FE0000} 66.3} & 67.4 & \multicolumn{1}{c|}{61.4} & {\color[HTML]{FE0000} 70.9} & \multicolumn{1}{c|}{\color[HTML]{FE0000} 62.7} & {\color[HTML]{FE0000} 73.4} & \multicolumn{1}{c|}{\color[HTML]{FE0000} 85.8} & 70.8 & \multicolumn{1}{c|}{\color[HTML]{FE0000} 77.4} & 69.7 & \multicolumn{1}{c|}{\color[HTML]{FE0000} 70.5} & 69.2 & \color[HTML]{FE0000} 70.7 \\
\hline\hline
\multicolumn{15}{c}{\textit{Open-source}} \\
\midrule
ToolLLaMA (ReAct) & 42.7 & \multicolumn{1}{c|}{36.2} & 35.4 & \multicolumn{1}{c|}{36.1} & 38.6 & \multicolumn{1}{c|}{34.6} & 39.9 & \multicolumn{1}{c|}{49.1} & 40.9 & \multicolumn{1}{c|}{38.7} & 29.8 & \multicolumn{1}{c|}{41.0} & 37.9 & 39.3 \\
ToolLLaMA (DFSDT) & 56.6 & \multicolumn{1}{c|}{39.9} & 55.5 & \multicolumn{1}{c|}{46.8} & 56.5 & \multicolumn{1}{c|}{41.8} & 49.7 & \multicolumn{1}{c|}{53.8} & 53.4 & \multicolumn{1}{c|}{49.2} & 53.6 & \multicolumn{1}{c|}{50.8} & 54.2 & 47.1 \\
ToolLLaMA (ReAct$\dag$) & 26.7 & \multicolumn{1}{c|}{22.1} & 25.0 & \multicolumn{1}{c|}{27.2} & 31.7 & \multicolumn{1}{c|}{29.4} & 23.1 & \multicolumn{1}{c|}{32.1} & 24.5 & \multicolumn{1}{c|}{28.2} & 20.5 & \multicolumn{1}{c|}{24.6} & 25.3 & 27.3 \\
ToolLLaMA (DFSDT$\dag$) & 41.8 & \multicolumn{1}{c|}{35.6} & 39.9 & \multicolumn{1}{c|}{37.3} & 44.9 & \multicolumn{1}{c|}{39.9} & 36.0 & \multicolumn{1}{c|}{47.2} & 39.1 & \multicolumn{1}{c|}{39.5} & 33.3 & \multicolumn{1}{c|}{26.2} & 39.2 & 37.6 \\
Ours & \underline{63.5} & \multicolumn{1}{c|}{\underline{52.1}} & \underline{64.2} & \multicolumn{1}{c|}{\underline{53.2}} & \underline{67.2} & \multicolumn{1}{c|}{\underline{54.2}} & \underline{62.1} & \multicolumn{1}{c|}{\underline{70.8}} & \underline{{\color[HTML]{FE0000} 71.9}} & \multicolumn{1}{c|}{\underline{65.3}} & \underline{67.5} & \multicolumn{1}{c|}{\underline{59.0}} & \underline{66.1} & \underline{59.1} \\
\bottomrule
\end{tabular}
}
\caption{A comparison of the performance of LLMs on StableToolBench. Considering that real-world APIs have time sensitivity, the experiments presented in the table are results that we reproduced during the period from September to October 2024. In this context, {\color[HTML]{FE0000} red} indicates the best result in the entire column, while \underline{underline} denotes the best result in the Open-source.}
\label{tab:main}
\end{table*}


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccccccc}
\hline
\textbf{Method} & \textbf{I1-Inst.} & \textbf{I1-Tool} & \textbf{I1-Cat.} & \textbf{I2-Inst.} & \textbf{I2-Cat.} & \textbf{I3-Inst.} & \textbf{Avg.} \\ \hline
ToolLLaMA (ReAct) & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
ToolLLaMA (DFSDT) & 2.24x & 2.58x & 2.57x & 2.82x & 3.26x & 2.61x & 2.67x \\
ToolLLaMA (ReAct$\dag$) & 1.59x & 1.43x & 2.69x & 1.44x & 1.37x & 1.76x & 1.69x \\
ToolLLaMA (DFSDT$\dag$) & 3.32x & 3.20x & 4.17x & 2.62x & 3.68x & 3.02x & 3.28x \\
Ours & 0.85x & 0.83x & 0.83x & 0.74x & 0.79x & 0.87x & 0.82x \\ \hline
\end{tabular}
}
\caption{The table presents a comparison of the inference times of LLMs. Using the average inference time of ToolLLaMA (CoT) as a benchmark, other LLMs are represented by corresponding multiples, labeled as x.}
\label{tab:time}
\end{table}

==> figures/max_step.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc|ccccccc}
\hline
\textbf{Method} &
   &
  \textbf{I1-Inst.} &
  \textbf{I1-Tool} &
  \textbf{I1-Cat.} &
  \textbf{I2-Inst.} &
  \textbf{I2-Cat.} &
  \textbf{I3-Inst.} &
  \textbf{Average} \\
\hline\hline
\multicolumn{9}{c}{\textit{GPT-series}} \\
\midrule 
                                     & Avg. & 4   & 4   & 4   & 5   & 5   & 5   & 5   \\
\multirow{-2}{*}{GPT-3.5 (CoT)}      & Max. & 7   & 8   & 8   & 8   & 8   & 8   & 8   \\ \hline
                                     & Avg. & 11  & 13  & 12  & 16  & 14  & 12  & 13  \\
\multirow{-2}{*}{GPT-3.5 (DFSDT)}    & Max. & 72  & 81  & 80  & 68  & 76  & 77  & 76  \\ \hline
                                     & Avg. & 25  & 26  & 26  & 31  & 31  & 38  & 30  \\
\multirow{-2}{*}{GPT-3.5 (parallel)} & Max. & 158 & 147 & 146 & 164 & 164 & 142 & 154 \\ \hline
                                     & Avg. & 3   & 3   & 3   & 4   & 3   & 4   & 3   \\
\multirow{-2}{*}{GPT-4 (CoT)}        & Max. & 9   & 13  & 12  & 12  & 12  & 12  & 12  \\ \hline
                                     & Avg. & 5   & 6   & 6   & 9   & 18  & 14  & 10  \\
\multirow{-2}{*}{GPT-4 (DFSDT)}      & Max. & 47  & 80  & 79  & 200 & 200 & 200 & 135 \\ \hline
                                     & Avg. & 4   & 12  & 12  & 3   & 5   & 10  & 8   \\
\multirow{-2}{*}{GPT-4 (parallel)}   & Max. & 36  & 200 & 200 & 20  & 88  & 130 & 112 \\
\hline\hline
\multicolumn{9}{c}{\textit{Open-source}} \\
\midrule 
                                     & Avg. & 3   & 3   & 3   & 3   & 3   & 3   & 3   \\
\multirow{-2}{*}{ToolLLaMA (CoT)}    & Max. & 4   & 5   & 4   & 4   & 4   & 4   & 4   \\ \hline
                                     & Avg. & 8   & 8   & 8   & 10  & 9   & 9   & 9   \\
\multirow{-2}{*}{ToolLLaMA (DFSDT)}  & Max. & 29  & 31  & 30  & 30  & 30  & 30  & 30  \\ \hline
                                     & Avg. & 3   & 3   & 3   & 3   & 3   & 3   & 3   \\
\multirow{-2}{*}{ToolLLaMA (COT*)}   & Max. & 4   & 5   & 4   & 4   & 4   & 4   & 4   \\ \hline
                                     & Avg. & 9   & 8   & 8   & 9   & 10  & 7   & 9   \\
\multirow{-2}{*}{ToolLLaMA (DFSDT*)} & Max. & 30  & 31  & 30  & 30  & 30  & 30  & 30  \\ \hline
                                     & Avg. & 2   & 2   & 2   & 2   & 2   & 2   & 2   \\
\multirow{-2}{*}{Ours}               & Max. & 19  & 15  & 14  & 10  & 7   & 6   & 12  \\ \hline
\end{tabular}
}
\caption{}
\label{tab:token}
\end{table*}

==> figures/token.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lc|cccccccccccccc@{}}
\toprule
\multicolumn{2}{l|}{} & \multicolumn{2}{c}{\textbf{I1-Inst.}} & \multicolumn{2}{c}{\textbf{I1-Tool}} & \multicolumn{2}{c}{\textbf{I1-Cat.}} & \multicolumn{2}{c}{\textbf{I2-Inst.}} & \multicolumn{2}{c}{\textbf{I2-Cat.}} & \multicolumn{2}{c}{\textbf{I3-Inst.}} & \multicolumn{2}{c}{\textbf{Average}} \\ \cmidrule(l){3-16} 
\multicolumn{2}{l|}{\multirow{-2}{*}{\textbf{Method}}} & C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} & C. & P. \\
\hline\hline
\multicolumn{16}{c}{\textit{GPT-series}} \\
\midrule 
GPT-3.5 (ReAct) &  & {\color[HTML]{FE0000} 0.3} & \multicolumn{1}{c|}{5.7} & {\color[HTML]{FE0000} 0.3} & \multicolumn{1}{c|}{7.2} & {\color[HTML]{FE0000} 0.2} & \multicolumn{1}{c|}{5.6} & {\color[HTML]{FE0000} 0.2} & \multicolumn{1}{c|}{7.9} & {\color[HTML]{FE0000} 0.2} & \multicolumn{1}{c|}{7.7} & {\color[HTML]{FE0000} 0.3} & \multicolumn{1}{c|}{9.7} & {\color[HTML]{FE0000} 0.3} & 7.3 \\
GPT-3.5 (DFSDT) &  & 1.1 & \multicolumn{1}{c|}{20.9} & 1.3 & \multicolumn{1}{c|}{27.9} & 1.2 & \multicolumn{1}{c|}{22.5} & 1.6 & \multicolumn{1}{c|}{34.6} & 1.4 & \multicolumn{1}{c|}{28.3} & 1.2 & \multicolumn{1}{c|}{26.2} & 1.3 & 26.7 \\
GPT-3.5 (Parallel) &  & 2.9 & \multicolumn{1}{c|}{42.8} & 3.2 & \multicolumn{1}{c|}{53.6} & 2.8 & \multicolumn{1}{c|}{42.7} & 3.3 & \multicolumn{1}{c|}{58.1} & 3..6 & \multicolumn{1}{c|}{59.6} & 4.5 & \multicolumn{1}{c|}{77.5} & 3.3 & 55.7 \\
GPT-4 (ReAct) &  & 0.4 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 4.3}} & 0.4 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 5.3}} & 0.4 & \multicolumn{1}{c|}{4.6} & 0.5 & \multicolumn{1}{c|}{6.1} & 0.5 & \multicolumn{1}{c|}{6.1} & 0.5 & \multicolumn{1}{c|}{7.5} & 0.5 & 5.7 \\
GPT-4 (DFSDT) &  & 0.8 & \multicolumn{1}{c|}{9.0} & 1.0 & \multicolumn{1}{c|}{13.5} & 0.9 & \multicolumn{1}{c|}{9.5} & 1.1 & \multicolumn{1}{c|}{17.5} & 1.5 & \multicolumn{1}{c|}{30.8} & 1.6 & \multicolumn{1}{c|}{30.4} & 1.2 & 18.5 \\
GPT-4 (Parallel) &  & 0.7 & \multicolumn{1}{c|}{6.0} & 1.2 & \multicolumn{1}{c|}{17.1} & 1.2 & \multicolumn{1}{c|}{18.7} & 0.7 & \multicolumn{1}{c|}{5.6} & 0.9 & \multicolumn{1}{c|}{9.7} & 1.4 & \multicolumn{1}{c|}{18.4} & 1.0 & 12.6 \\
\hline\hline
\multicolumn{16}{c}{\textit{Open-source}} \\
\midrule
ToolLLaMA (ReAct) &  & 0.6 & \multicolumn{1}{c|}{6.4} & 0.5 & \multicolumn{1}{c|}{7.1} & 0.5 & \multicolumn{1}{c|}{5.8} & 0.6 & \multicolumn{1}{c|}{7.8} & 0.6 & \multicolumn{1}{c|}{7.4} & 0.6 & \multicolumn{1}{c|}{8.5} & 0.6 & 7.2 \\
ToolLLaMA (DFSDT) &  & 1.3 & \multicolumn{1}{c|}{19.6} & 1.4 & \multicolumn{1}{c|}{22.7} & 1.2 & \multicolumn{1}{c|}{18.2} & 1.5 & \multicolumn{1}{c|}{27.8} & 1.5 & \multicolumn{1}{c|}{26.9} & 1.4 & \multicolumn{1}{c|}{23.8} & 1.4 & 23.2 \\
ToolLLaMA (ReAct$\dag$) &  & 0.5 & \multicolumn{1}{c|}{6.7} & 0.5 & \multicolumn{1}{c|}{7.2} & \underline{0.4} & \multicolumn{1}{c|}{5.9} & 0.5 & \multicolumn{1}{c|}{7.8} & \underline{0.4} & \multicolumn{1}{c|}{7.6} & \underline{0.4} & \multicolumn{1}{c|}{8.2} & 0.5 & 7.2 \\
ToolLLaMA (DFSDT$\dag$) &  & 1.3 & \multicolumn{1}{c|}{25.1} & 1.3 & \multicolumn{1}{c|}{24.3} & 1.1 & \multicolumn{1}{c|}{19.7} & 1.2 & \multicolumn{1}{c|}{24.1} & 1.3 & \multicolumn{1}{c|}{29.6} & 1.0 & \multicolumn{1}{c|}{19.4} & 1.2 & 23.7 \\
Ours &  & \underline{0.5} & \multicolumn{1}{c|}{\underline{4.8}} & \underline{0.5} & \multicolumn{1}{c|}{\underline{5.4}} & 0.5 & \multicolumn{1}{c|}{\underline{{\color[HTML]{FE0000} 4.6}}} & \underline{0.5} & \multicolumn{1}{c|}{{\underline{\color[HTML]{FE0000} 5.1}}} & 0.5 & \multicolumn{1}{c|}{{\underline{\color[HTML]{FE0000} 5.0}}} & 0.5 & \multicolumn{1}{c|}{\underline{\color[HTML]{FE0000} 6.3}} & \underline{0.5} & \underline{{\color[HTML]{FE0000} 5.2}} \\ \bottomrule
\end{tabular}
}
\caption{The table shows the performance of various LLMs in terms of token consumption. All values in the table are expressed in thousands. On the horizontal axis, C. stands for \textit{Completion} and P. for \textit{Prompt}. On the vertical axis, Avg. indicates average and Max. represents the maximum. Similarly, {\color[HTML]{FE0000} red} indicates the best result in the entire column, while \underline{underline} denotes the best result in the open-source.}
\label{tab:token}
\end{table*}
